High-Energy Neutrino and Gamma Ray Production in Clusters of Galaxies

We compute the contribution from clusters of galaxies to the diffuse neutrino and $\gamma-$ray background. Due to their unique magnetic-field configuration, cosmic rays (CRs) with energy $\leq10^{17}$ eV can be confined within these structures over cosmological time scales, and generate secondary particles, including neutrinos and $\gamma-$rays, through interactions with the background gas and photons. We employ three-dimensional (3D) cosmological magnetohydrodynamical (MHD) simulations of structure formation to model the turbulent intergalactic and intracluster media. We propagate CRs in these environments using multi-dimensional Monte Carlo simulations across different redshifts (from $z \sim 5$ to $z = 0$), considering all relevant photohadronic, photonuclear, and hadronuclear interactions. We also include the cosmological evolution of the CR sources. We find that for CRs injected with a spectral index $1.5 - 2.7$ and cutoff energy $E_\text{max} = 10^{16} - 10^{17}$~eV, clusters contribute to a substantial fraction to the diffuse fluxes observed by the IceCube and Fermi-LAT, and most of the contribution comes from clusters with $M > 10^{14} \, M_{\odot}$ and redshift $z < 0.3$. We also estimated the multimessenger contributions from the local galaxy cluster.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

